LibriS2S: A German-English Speech-to-Speech Translation Corpus

Recently, we have seen an increasing interest in the area of speech-to-text translation. This has led to astonishing improvements in this area. In contrast, the activities in the area of speech-to-speech translation is still limited, although it is essential to overcome the language barrier. We believe that one of the limiting factors is the availability of appropriate training data. We address this issue by creating LibriS2S, to our knowledge the first publicly available speech-to-speech training corpus between German and English. For this corpus, we used independently created audio for German and English leading to an unbiased pronunciation of the text in both languages. This allows the creation of a new text-to-speech and speech-to-speech translation model that directly learns to generate the speech signal based on the pronunciation of the source language. Using this created corpus, we propose Text-to-Speech models based on the example of the recently proposed FastSpeech 2 model that integrates source language information. We do this by adapting the model to take information such as the pitch, energy or transcript from the source speech as additional input.

==> 03fastspeech2.tex <==
In the TTS pipeline two models are used. A feature generation model takes the phoneme sequence of the target sentence as input and outputs the Mel Frequency Cepstral Coefficients (MFCCs). The second model, called the vocoder, takes in these MFCCs as input and outputs the generated speech in waveform.\\

The feature generation model used for this research is FastSpeech 2\cite{ren2021fastspeech}. This model is of particular interest because it has separate predictors for pitch and energy as can be seen in Fig. \ref{fig:fs2arch}. The implementation used in this research can be found in the TensorFlowTTS\footnote{https://github.com/TensorSpeech/TensorFlowTTS} GitHub repository. Compared to the original paper, this implementation has made a few changes such as: 1) The pitch and energy are predicted per phoneme and not on the frame level. 2) The pitch and energy are normalized using the z-score and these are being predicted. 3) A post-net similar to the one used by the Tacotron 2 \cite{shen2018natural} paper is being used to ``predict a residual to add to the prediction to improve the overall reconstruction"\cite{shen2018natural} is implemented.\\
The vocoder model used in this research is a Multi-band MelGAN \cite{yang2020multiband}. This model is implemented in the same GitHub repository but its implementation will not be discussed.


